Information Bottleneck Methods for Distributed Learning

We study a distributed learning problem in which Alice sends a compressed distillation of a set of training data to Bob, who uses the distilled version to best solve an associated learning problem. We formalize this as a rate-distortion problem in which the training set is the source and Bob's cross-entropy loss is the distortion measure. We consider this problem for unsupervised learning for batch and sequential data. In the batch data, this problem is equivalent to the information bottleneck (IB), and we show that reduced-complexity versions of standard IB methods solve the associated rate-distortion problem. For the streaming data, we present a new algorithm, which may be of independent interest, that solves the rate-distortion problem for Gaussian sources. Furthermore, to improve the results of the iterative algorithm for sequential data we introduce a two-pass version of this algorithm. Finally, we show the dependency of the rate on the number of samples $k$ required for Gaussian sources to ensure cross-entropy loss that scales optimally with the growth of the training set.

==> batch_data.tex <==
%!TEX root = main.tex
\section{Batch dataset}\label{sect:batch.dataset}
To find $R^{k}_{\text{B}}(D)$, we leverage the equivalence between this rate-distortion problem and the information bottleneck over the Markov chain $X-\theta-X^k-T$. This translates the rate-distortion problem to finding the conditional distribution $p(t|x^k)$ that solves the problem
\begin{equation}\label{eqn:unsupervised.ib}
  \min_{p(t|x^k)} \mathcal{L}=I(X^k;T)-\beta I(X;T),
\end{equation} 
where $I(X^k;T)$ determines the rate, $I(X;T) = H(X) - H(X|T)$ determines the average distortion, and $\beta$ determines the trade-off between the two and dictates which point on the rate-distortion curve the solution will achieve. For discrete sources, one can use the iterative method proposed in \cite{tishby2000information} to solve (\ref{eqn:unsupervised.ib}). This method only guarantees a {\em local} optimum, but it performs well in practice. When $\theta$ and $X$ are jointly Gaussian, one can use the results in \cite{chechik2005information} for the {\em Gaussian} information bottleneck, in which the optimum $p(t|x^k)$ is Gaussian and given by a noisy linear compression of the source.

%Machine learning problem motivates us to define the distortion as the {\em cross-entropy} loss where it is closely related to the KL divergence between the two distributions, and the Kullback-Liebler (KL) divegence is an usual metric of the relevant content in the machine learning problem. In other words, in the simple prediction problem, we encode the estimated $\theta$ using the alphabet $\mathcal{T}$, and the distortion metric shows how much information we obtain from the encoder. As a result, this problem can be solved by IB method, which extracts the relevant information from $\theta$ to predict the $X$ \cite{Tishby}, as follows:
% \begin{equation}
% \min_{p(t|\theta)} \mathcal{L}: \mathcal{L}=I(\theta;T)-\beta I(T;X)
% \end{equation} 
% subject to the $X\mbox{-}\theta\mbox{–}T$, and $I(\theta;T)$ is the rate. $I(T;X)$ denotes the relevant information and it is $I(T;X)=H(X)-H(X|T)$, where $H(T|X)$ is the distortion. Therefore, by maximizing the relevant information we minimize the $D$.\par
% We employ the IB method \cite{Tishby} to compute the following probabilities in order to draw the distortion-rate curve in Fig.~\ref{fig:RD_dis} for discrete value of $X,\theta$ and $T$:
% \begin{align*}
% &q^{(n)}(t|\theta)=\frac{q^{(n)}(t)}{Z^{(n)}(\theta,\beta)}\exp\left[-\beta D_{KL}\left[p(x|\theta)||p(x|t)\right]\right]\\
% &q^{(n+1)}(t)=\sum_{\theta}q^{(n)}(t|\theta)p(\theta)\\
% &q^{(n+1)}(x|t)=\frac{1}{q^{(n)}(t)}\sum_{\theta}q^{(n)}(t|\theta)p(\theta,x)
% \end{align*}
% where the $q^{(n)}(t|\theta)$, $q^{(n)}(t)$ and $q^{(n+1)}(x|t)$ are normalized distributions, and the number of iterations is denoted by $n$.
% In Figure \ref{fig:simple.unsupervised} we plot $R^{\infty}_{\text{U}}(D)$ for discrete and Gaussian sources. In Figure \ref{fig:simple.unsupervised.discrete}, $X$ is binary and $|\Theta| = 6$, with the joint distribution expressed as a $2 \times 8$ matrix:
% \begin{equation*}
% p(x,\theta)=
% \begin{bmatrix}
%   0.25 & 0.15 & 0.06 & 0.04 & 0.015 & 0.01 \\
%   0.01 & 0.015 & 0.02 & 0.03 & 0.15 & 0.25
% \end{bmatrix}.
% \end{equation*}
% In Figure \ref{fig:simple.unsupervised.gaussian}, we let $p(x|\theta) = \mathcal{N}(\theta, \Sigma)$ and $p(\theta) = \mathcal{N}(0,XXX)$ [PARINAZ: What are the dimensions of the random vectors $x$ and $\theta$? What value of $\Sigma$ is chosen? What is the covariance of $\theta$?]
% % We employ the IB method \cite{Tishby} to compute the following probabilities in order to draw the distortion-rate curve in Fig.~\ref{fig:RD_dis} for discrete value of $X,\theta$ and $T$:
% \begin{figure}[htb]
%   \centering
%   \begin{subfigure}{0.4\textwidth}
%     \includegraphics[width=\textwidth]{IB_dis_RD.pdf}
%    \caption{Discrete $X,\theta$.}
%     \label{fig:logistic.regression.rho.1}
%    \end{subfigure}
%      \begin{subfigure}{0.4\textwidth}
%     \includegraphics[width=\textwidth]{Rate_dis_Gaussian.pdf}
%     \caption{Jointly Gaussian $X,\theta$}
%     \label{fig:simple.unsupervised.gaussian}
%    \end{subfigure}
%    \caption{Rate-distortion curves for ``simple'' unsupervised learning.}
%   \label{fig:simple.unsupervised}
% \end{figure}

% Fig.~\ref{fig:RD_Gaus} shows the distortion-rate curve for continuous $X,\theta$ and $T$.
% \begin{figure}[htbp]
% \centering
%   \includegraphics[height=5.5cm, width=7.5cm]{IB_dis_RD.pdf}
% \caption {Distortion Rate curve for discrete value of $X,\theta$ and $T$, where 
% $p(x,\theta)=[0.25,0.01;0.15,0.015;0.06,0.02;0.04,0.03;0.015,0.15;0.01,0.25]; $.}
% \label{fig:RD_dis}
% \end{figure}
% \begin{figure}[htbp]
% \centering
%   \includegraphics[height=5.5cm, width=7.5cm]{Rate_dis_Gaussian.pdf}
% \caption {Distortion Rate curve for jointly Gaussian distribution of $(X,\theta)\sim\mathcal{N}(0,\Sigma)$, where $\Sigma$ selected randomly.}
% \label{fig:RD_Gaus}
% \end{figure}
%Observe that in the Fig.~\ref{fig:RD_dis} and Fig.~\ref{fig:RD_Gaus} the distortion value converges the bounds that we found in the Section \ref{sect:problem.statement}. [PARINAZ: Is this true? How can I see this just from looking at the plots?]
%\begin{align*}
%R(D)=I(\theta;T)\geq I(X;T)&=H(X)-H(X|T)\\
%&=H(X)-D
%\end{align*}
%where $D$ is the distortion value. The above expression shows that for each value of the distortion the rate can not be less that $H(X)-D$.\par 
%\subsection{$k$-sample Unsupervised Learning}
%To find $R^{k}_{\text{U}}(D)$, we can make use of similar analogies with the information bottleneck over the Markov chain $X - X^k - T$. 
%However, a naive implementation of the methods from \cite{tishby2000information,chechik2005information} imposes high computational and storage burdens. One can reduce those burdens by exploiting the fact that $X$ and $X^k$ are i.i.d. samples drawn from $p(x|\theta)$.

\subsubsection{Discrete Source}
For $k$-sample with a discrete source, when $X$ and $X^k$ are i.i.d. samples drawn from $p(x|\theta)$, the histogram $H_k$ of $X^k$ is a sufficient statistic for $\theta$, and we compute $p(x^k)$, $p(x|X^k)$ and $p(x,x^k)$ in terms of the histogram. Then, the iterative IB algorithm proposed in \cite{tishby2000information}, can be rewritten
%For discrete $X$, the iterative IB algorithm proposed in \cite{tishby2000information} has the following iterations applied to the Markov chain $X-X^k-T$:
\begin{align*}
  q^{(n)}(t|H_k) &= \frac{q^{(n)}(t)}{Z^{(n)}(H_k,\beta)}\exp\left[-\beta D_{KL}\left[p(x|H_k)||p(x|t)\right]\right]\\
  q^{(n+1)}(t) &= \sum_{\theta}q^{(n)}(t|H_k)p(H_k)\\
  q^{(n+1)}(x|t) &= \frac{1}{q^{(n)}(t)}\sum_{\theta}q^{(n)}(t|H_k)p(H_k,x),
\end{align*} 
%\begin{align*}
%  q^{(n)}(t|x^k) &= \frac{q^{(n)}(t)}{Z^{(n)}(x^k,\beta)}\exp\left[-\beta D_{KL}\left[p(x|x^k)||p(x|t)\right]\right]\\
%  q^{(n+1)}(t) &= \sum_{\theta}q^{(n)}(t|x^k)p(x^k)\\
%  q^{(n+1)}(x|t) &= \frac{1}{q^{(n)}(t)}\sum_{\theta}q^{(n)}(t|x^k)p(x^k,x),
%\end{align*} 
where $n$ is the iteration index, $q^{(n)}(t|x^k)$ is the choice for $p(t|x^k)$ at iteration $n$, and the other iterated distributions $q^{(n)}(t),q^{(n)}(x|t)$ are intermediate distributions. The number of terms in the distribution $q^{(n)}(t|x^k)$ is upper bounded to $|\mathcal{T}|k^{|\mathcal{X}|-1}$ entries by using the histogram of $X^k$. This distribution must be updated every iteration, and computing the distributions $q^{(n+1)}(t)$ and $q^{(n+1)}(x|t)$ requires summing over $q^{(n)}(t|x^k)$, $p(x^n)$, and $p(x^k,x)$, the latter two of which are computed based on the histogram and have at most $|\mathcal{T}|\cdot k^{|\mathcal{X}| - 1}$, $k^{|\mathcal{X} - 1|}$ entries, respectively. Standard cardinality bounds would suggest that $|\mathcal{T}| = \min\{|\Theta| , k^{|\mathcal{X}| - 1}\}$ is sufficient to achieve $R^{k}_{\text{B}}(D)$. This bound on $\mathcal{T}$ is established along with a fact that $T$ depends on $X^k$ only through $\theta$. 
%\begin{prop}
%  For $k$-sample unsupervised learning with a discrete source, $|\mathcal{T}| = \min\{|\Theta| , k^{|\mathcal{X}| - 1}\} + 1$ is sufficient to achieve $R^{k}_{\text{B}}(D)$. Furthermore, $q^{(n)}(t|x^k)$, $p(x^k)$, and $p(x^k,x)$ can be represented by no more than $|\mathcal{T}|\cdot k^{|\mathcal{X} - 1|}$, $k^{|\mathcal{X} - 1|}$, and $|\mathcal{X}| \cdot k^{|\mathcal{X} - 1|}$ terms, respectively.
%\end{prop}
%\begin{IEEEproof}[Proof sketch]
% Because the training points are drawn i.i.d., the distributions involving $X^k$ are invariant to permutations. Consequently, one can express the distributions in terms of the {\em histogram} of $X^k$; the histogram of $X^k$ is a sufficient statistic for $p(x|X^k)$, which bounds the number of terms in the distribution. This fact also, along with the fact that $T$ depends on $X^k$ only through $\theta$, establishes the bound on $|\mathcal{T}|$.
%\end{IEEEproof}
As a result, the problem structure allows one to reduce the complexity of the IB algorithm from exponential to polynomial when $|\mathcal{X}|$ is constant, albeit of a potentially large degree.
%\setlength\belowcaptionskip{-4ex}
\begin{figure}[H]
\centering
  \includegraphics[width=7cm]{IB_Discrete.pdf}
\caption {Rate-distortion curve for Bernoulli distribution with uniform prior and $k\in\{4,10,20,50\}$.}
\label{fig:Rate-Discrete}
\end{figure}
In Figure~\ref{fig:Rate-Discrete} we plot the rate-distortion curve for a Bernoulli distribution with a uniform prior and $|\mathcal{T}|=k+1$ is sufficient for the Bernoulli distribution. As the number of samples increase we see that the cross entropy loss decreases; however, the cross entropy loss for each sample is bounded by $H(X|X^k)$.
\subsubsection{Gaussian Source}
When $X,\theta$ are jointly (multivariate) Gaussian, one can appeal to the Gaussian information bottleneck, \cite{chechik2005information}, where it is shown that the optimum $T$ is a noisy linear projection of the source, which one can find iteratively or in closed form. If $X$ is a $d$-dimensional multivariate Gaussian, however, naive application of this approach requires one to find an $dk \times dk$ projection matrix. Here again, exploitation of the structure of this problem simplifies the result.

Without loss of generality, let $p(x|\theta) = \mathcal{N}(\theta,\Sigma_x)$ and $p(\theta) = \mathcal{N}(0,\Sigma_\theta)$, where $\Sigma_x \in \mathbb{R}^{d \times d}$ is the covariance of the data, and $\Sigma_\theta$ is the covariance of the prior. For the general problem with the Markov chain $Y - \theta - X - T$,  For $k$-sample training set $X^k$ with a Gaussian source, the sample mean, $S_k=\frac{1}{k}\sum_{i=1}^k x_i$ is a sufficient statistic for $\theta$ and we have the Markov chain $X - \theta - S_k - T$.   \cite{chechik2005information} shows that the IB-optimum compression is $T = AS_k + Z$, where $Z$ is white Gaussian noise and $A$ is a matrix whose rows are scaled left eigenvectors of the matrix
\begin{equation*}
  K = \frac{\Sigma_x+\Sigma_{\theta}}{k}+\frac{k-1}{k}\Sigma_{\theta} - \Sigma_\theta (\Sigma_{x} + \Sigma_\theta)^{-1}\Sigma_\theta.
\end{equation*}
Specifically, let $\lambda_1,\lambda_2,\dots$ be the ascending eigenvalues of $K$ and $v_1,v_2$ be the associated left eigenvectors. For $\beta>1$, only the eigenvectors $v_i$ such that $\beta_i := (1-\lambda_i)^{-1} < \beta$ are incorporated into $A$, and the resulting rate-distortion point is given parametrically by
\begin{align*}
  R(\beta) &= \frac{1}{2}\sum_{i=1}^{n(\beta)} \log\left((\beta-1)\frac{1-\lambda_i}{\lambda_i} \right) \\
  D(\beta) &= \frac{1}{2}\sum_{i=1}^{n(\beta)} \log\left(\lambda_i \frac{\beta}{\beta - 1}\right) + h(X),
\end{align*}
where $n(\beta)$ is the number of eigenvalues satisfying $\beta_i < \beta$. For $\beta \approx 1$, the rate is small and the distortion is close to the maximum value $h(X)$; as $\beta \to \infty$ the rate becomes large and the distortion converges to $h(X|X^k)$.

The problem setting implies structure on the compression matrix $A$ beyond what is obvious from above.
%\begin{theorem}
%  The rank of $K$ is at most $d$, and the left eigenvectors of $K$ are the left eigenvectors of the matrix $\Sigma_\theta(\Sigma_x + \Sigma_\theta)^{-1}$.
%\end{theorem}
%This result follows from the sufficiency of the sample mean $S_k$. Its implication is that, regardless of $k$, the optimum compression is a $d$-dimensional representation of the  training set $X^k$; further, one can preprocess $X^k$ to its sample mean before apply the compression. Rather than finding a $dk$-dimensional operator in general, in this case one can derive the optimum operator from the $d$-dimensional matrix $\Sigma_\theta(\Sigma_x + \Sigma_\theta)^{-1}$ and the computation of the $d$ eigenvalues of $K$.
%\setlength\belowcaptionskip{-2ex}
\begin{figure}[H]
\centering
  \includegraphics[width=7cm]{GIB_DifferentNumebrofSamples.pdf}
\caption {Rate-distortion curve for jointly Gaussian distribution with $d=6$ and $k\in\{5,20,100,200,500\}$.}
\label{fig:Rate-Dist}
\end{figure}
%%%%%%
% \begin{theorem}
% The eigenvector of the $ \Sigma_{x^kx}\Sigma_x^{-1}\Sigma_{xx^k}\Sigma_{x^k}^{-1}$ is the combination of the eigenvector of the $\Sigma Q$.
% \end{theorem}
% \begin{proof}
% As it is represented in the (\ref{Rate}) and (\ref{bottleneck}) the GIB is function of $\beta$ and $\lambda$. Therefore, the eigenvalues of the $\Sigma_{x^k|x}\Sigma_{x^n}^{-1}$ is important for us. Based on the (\ref{x^n}), $\Sigma_{x^n|x}\Sigma_{x^n}^{-1}$ can be written as:
% \begin{align*}
% &\Sigma_{x^k|x}\Sigma_{x^n}^{-1}=I-\Sigma_{x^kx}\Sigma_x^{-1}\Sigma_{xx^k}\Sigma_{x^n}^{-1}\\
% &\Sigma_{xx^k}=\begin{bmatrix}
%     \Sigma_{\theta} & \Sigma_{\theta}  & \dots & \Sigma_{\theta} 
% \end{bmatrix}
% \end{align*}
% Therefore, by assuming $Q=(\Sigma_x+\Sigma_{\theta})^{-1}$ and $\Sigma=\Sigma_{\theta}$ we can rewrite the $\Sigma_{x^nx}\Sigma_x^{-1}\Sigma_{xx^n}\Sigma_{x^n}^{-1}$ as
% \begin{equation}
% \begin{bmatrix}
%     \Sigma Q\Sigma       & \Sigma Q\Sigma  & \dots & \Sigma Q\Sigma \\
%     \Sigma Q\Sigma       & \Sigma Q\Sigma  & \dots & \Sigma Q\Sigma \\
%     \hdotsfor{4} \\
%     \Sigma Q\Sigma       & \Sigma Q\Sigma  & \dots & \Sigma Q\Sigma
% \end{bmatrix}
% \times 
% \Sigma_{x^n}^{-1}
% \end{equation}
% Then,
% \begin{align*}
% &\Sigma_{x^k}=\begin{bmatrix}
%     U       & V^T  \\
%     V       & Q^{-1}  \\
% \end{bmatrix}, \\ 
% &\Sigma_{x^k}^{-1}=\begin{bmatrix}
%   (U-V^TQV)^{-1}   & -U^{-1}V^T(Q^{-1}-VV^T)  \\
%    -U^{-1}V^T(Q^{-1}-VV^T)  & (Q^{-1}-V^TQV)^{-1}  \\
% \end{bmatrix}\\
% &(U-V^TQV)^{-1}=(I+\sum_{i=1}^\infty(UV^TQV)^i)U^{-1} 
% \end{align*}
% where $U$ is the combination of $Q$ and $\Sigma$. Moreover, $V=\Sigma\times 1_{n\times 1}$.
% \end{proof}
% Based on our experimental results, the maximum number of the eigenvalues that we use for computing the GIB curve $n_\beta$ is the same for constant $Rate$ with different $k$ (number of samples).\par
In Figure~\ref{fig:Rate-Dist} we plot the rate-distortion curve for a Gaussian source, where $d=6$ and the covariances are drawn elementwise at random from the standard normal distribution and symmetrized. The curve is smooth because the Gaussian information bottleneck provides an exactly optimum solution.
% \begin{align*}
% h(x|x^k)-h(x|\theta)=D_{KL}\left(p(x|x^k)||p(x|t)\right)
% \end{align*}
% Fig.~\ref{fig:Rate-Sample} illustrate that by choosing the rate function as a polynomial $\log(k)$, where $k$ is the number of samples, difference between the distortion function $h(x|t)$ and $h(x|\theta)$ falls down with $1\mathbin{/}k$.
% Note that the KL-Divergence also falls down with $1\mathbin{/}k$. In conclusion, as the number of samples increases this difference $D-h(x|\theta)$ and KL-Divergence converges to each other. \par
% \begin{figure}[htbp]
% \centering
%   \includegraphics[height=5.5cm, width=7.5cm]{Rate_Samples.pdf}
% \caption {Relation between rate function and number of samples.}
% \label{fig:Rate-Sample}
% \end{figure}
% \begin{prop}\label{prpp:cardinality} Based on the Caratheodory theorem in n-letter prediction problem, $|\mathcal{T}|\leq |\mathcal{X}^k|+1$. This upper bound is linearly increase by the number of samples; however, for the discrete value of $\theta$ we can find a tighter cardinality bound.
% \begin{align}
% &R(D)=I(T;X^k)\geq I(T;\theta)\nonumber\\
% &|\mathcal{T}|\leq |\mathcal{\theta}|+1
% \end{align}
%  \end{prop} 

%  \subsection{Experimental Results}
%  In this part, we study empirically the distortion-rate curve of prediction for binary Restricted Boltzmann Machines (RBMs). First, consider the setting shown in Fig.~\ref{fig:Deep_RBM} with two neurons in the visible and hidden layers with one hidden layer. Similar to how IB method used in the discrete distribution to obtain the distortion-rate curve, we use the IB method for (RBMs). In the Fig.~\ref{fig:Dis_RBM}, we assume this structure, $X \mbox{–} \theta \mbox{–} T$, where $\theta$ is the parameters of the RBMs consists of weights and biases between visible and hidden layers, and they are selected from $\mathcal{N}(0,1)$. Two different discrete values for $\theta$ are considered in this scenario. As it is shown in Fig.~\ref{fig:Dis_RBM} the distortion $H(X|T)$ is decrease by increasing the rate $I(T;\theta)$. \\    
% \begin{figure}[htbp]
% \centering
%   \includegraphics[height=5.5cm, width=7.5cm]{IB_dis_RBM.pdf}
% \caption {Distortion-rate curve for different values of $\theta$.}
% \label{fig:Dis_RBM}
% \end{figure}    
% Now consider the continuous $\theta$ and this structure $X\mbox{-}\theta\mbox{-}X^n\mbox{–}T$, based on the \cite{Sankar privacy} and the Caratheodory theorem cardinality of the $T$ is bounded by $|\mathcal{X}_k|+1$. However, based on our experimental results even by choosing smaller cardinality for $T$ we can reach to the specific value for rate and distortion. We show the distortion-rate curve for this scenario and $|\mathcal{T}|=|\mathcal{X}_k|$, in Fig.~\ref{fig:Cos_RBM_xk}, for $|\mathcal{T}|=|\mathcal{X}|$, where  we see the distortion increases for a fix value of rate. 
% \begin{figure}[htbp]
% \centering
%   \includegraphics[height=5.5cm, width=7.5cm]{IB_con_RBM_Xk.pdf}
% \caption {Distortion-Rate curve for continuous $\theta$.}
% \label{fig:Cos_RBM_xk}
% \end{figure}
% \begin{figure}[htbp]
% \centering
%   \includegraphics[height=5.5cm, width=7.5cm]{IB_con_RBM_X.pdf}
% \caption {Distortion-Rate curve for continuous $\theta$.}
% \label{fig:Cos_RBM_x}
% \end{figure}

==> results.tex <==
%!TEX root = main.tex
\section{results_batch}\label{results}
%In this section we explore the results for both {\em batch}, in which we observe a set of $k$ i.i.d. samples at one time and {\em stream data}, in which data comes one-by-one in each round of the data transmission.
In this section, for both {\em batch} and {\em stream data}, we examine both {\em fundamental limits} and {\em algorithmic method} to find a compressed representation of the observed random variables. 
%First, we consider the {\em batch data}, in which $k$ i.i.d. samples are observed at one time. Second, we explore two approaches to solve the streaming problem, where data comes one-by-one in each round of the data transmission.    
\subsection{Batch Data}
First, we consider the {\em batch data}, in which $k$ i.i.d. samples are observed at one time. In this setting, we analyze both discrete and continuous distributions, in terms of the fundamental limits and algorithmic method. 
\subsubsection{Fundamental Limits}
To find $D^{k}_{\text{B}}(R)$, we leverage the equivalence between this distortion-rate problem and the information bottleneck over the Markov chain $X-\theta-X^k-T$. Considering $I(X;T)=H(X)-H(X|T)$ and solving the distortion-rate problem by Lagrange multiplier translates the distortion-rate problem to finding the conditional distribution $p(t|x^k)$ that solves the problem
\begin{equation}\label{eqn:unsupervised.ib}
  \min_{p(t|x^k)} \mathcal{L}=I(X^k;T)-\beta I(X;T),
\end{equation} 
where $I(X^k;T)$ determines the rate, $I(X;T) = H(X) - H(X|T)$ determines the average distortion, and $\beta$ determines the trade-off between the two and dictates which point on the rate-distortion curve the solution will achieve. For {\em discrete} sources, one can use the iterative method proposed in \cite{tishby2000information} to solve (\ref{eqn:unsupervised.ib}). This method only guarantees a {\em local} optimum, but it performs well in practice. When $\theta$ and $X$ are jointly Gaussian, one can use the results in \cite{chechik2005information} for the {\em Gaussian} information bottleneck, in which the optimum $p(t|x^k)$ is Gaussian and given by a noisy linear compression of the source.
\subsubsection*{Discrete Source}
For $k$-sample with a discrete source, when $X$ and $X^k$ are i.i.d. samples drawn from $p(x|\theta)$, the histogram $H_k$ of $X^k$ is a sufficient statistic for $\theta$, and similar to \cite[Theorem.1]{tishby2000information} the optimum mapping $p(t|x^k)$ that minimize (\ref{eqn:unsupervised.ib}) is computed as:
\begin{equation}
  q(t|H_k) = \frac{q(t)}{Z(H_k,\beta)}\exp\left[-\beta D_{KL}\left[p(x|H_k)||p(x|t)\right]\right],
\end{equation} 
where $Z(H_k,\beta)$ is the normalization function and $\beta$ is the Lagrangian multiplier in equation \ref{eqn:unsupervised.ib}.
%Machine learning problem motivates us to define the distortion as the {\em cross-entropy} loss where it is closely related to the KL divergence between the two distributions, and the Kullback-Liebler (KL) divegence is an usual metric of the relevant content in the machine learning problem. In other words, in the simple prediction problem, we encode the estimated $\theta$ using the alphabet $\mathcal{T}$, and the distortion metric shows how much information we obtain from the encoder. As a result, this problem can be solved by IB method, which extracts the relevant information from $\theta$ to predict the $X$ \cite{Tishby}, as follows:
% \begin{equation}
% \min_{p(t|\theta)} \mathcal{L}: \mathcal{L}=I(\theta;T)-\beta I(T;X)
% \end{equation} 
% subject to the $X\mbox{-}\theta\mbox{–}T$, and $I(\theta;T)$ is the rate. $I(T;X)$ denotes the relevant information and it is $I(T;X)=H(X)-H(X|T)$, where $H(T|X)$ is the distortion. Therefore, by maximizing the relevant information we minimize the $D$.\par
% We employ the IB method \cite{Tishby} to compute the following probabilities in order to draw the distortion-rate curve in Fig.~\ref{fig:RD_dis} for discrete value of $X,\theta$ and $T$:
% \begin{align*}
% &q^{(n)}(t|\theta)=\frac{q^{(n)}(t)}{Z^{(n)}(\theta,\beta)}\exp\left[-\beta D_{KL}\left[p(x|\theta)||p(x|t)\right]\right]\\
% &q^{(n+1)}(t)=\sum_{\theta}q^{(n)}(t|\theta)p(\theta)\\
% &q^{(n+1)}(x|t)=\frac{1}{q^{(n)}(t)}\sum_{\theta}q^{(n)}(t|\theta)p(\theta,x)
% \end{align*}
% where the $q^{(n)}(t|\theta)$, $q^{(n)}(t)$ and $q^{(n+1)}(x|t)$ are normalized distributions, and the number of iterations is denoted by $n$.
% In Figure \ref{fig:simple.unsupervised} we plot $R^{\infty}_{\text{U}}(D)$ for discrete and Gaussian sources. In Figure \ref{fig:simple.unsupervised.discrete}, $X$ is binary and $|\Theta| = 6$, with the joint distribution expressed as a $2 \times 8$ matrix:
% \begin{equation*}
% p(x,\theta)=
% \begin{bmatrix}
%   0.25 & 0.15 & 0.06 & 0.04 & 0.015 & 0.01 \\
%   0.01 & 0.015 & 0.02 & 0.03 & 0.15 & 0.25
% \end{bmatrix}.
% \end{equation*}
% In Figure \ref{fig:simple.unsupervised.gaussian}, we let $p(x|\theta) = \mathcal{N}(\theta, \Sigma)$ and $p(\theta) = \mathcal{N}(0,XXX)$ [PARINAZ: What are the dimensions of the random vectors $x$ and $\theta$? What value of $\Sigma$ is chosen? What is the covariance of $\theta$?]
% % We employ the IB method \cite{Tishby} to compute the following probabilities in order to draw the distortion-rate curve in Fig.~\ref{fig:RD_dis} for discrete value of $X,\theta$ and $T$:
% \begin{figure}[htb]
%   \centering
%   \begin{subfigure}{0.4\textwidth}
%     \includegraphics[width=\textwidth]{IB_dis_RD.pdf}
%    \caption{Discrete $X,\theta$.}
%     \label{fig:logistic.regression.rho.1}
%    \end{subfigure}
%      \begin{subfigure}{0.4\textwidth}
%     \includegraphics[width=\textwidth]{Rate_dis_Gaussian.pdf}
%     \caption{Jointly Gaussian $X,\theta$}
%     \label{fig:simple.unsupervised.gaussian}
%    \end{subfigure}
%    \caption{Rate-distortion curves for ``simple'' unsupervised learning.}
%   \label{fig:simple.unsupervised}
% \end{figure}

% Fig.~\ref{fig:RD_Gaus} shows the distortion-rate curve for continuous $X,\theta$ and $T$.
% \begin{figure}[htbp]
% \centering
%   \includegraphics[height=5.5cm, width=7.5cm]{IB_dis_RD.pdf}
% \caption {Distortion Rate curve for discrete value of $X,\theta$ and $T$, where 
% $p(x,\theta)=[0.25,0.01;0.15,0.015;0.06,0.02;0.04,0.03;0.015,0.15;0.01,0.25]; $.}
% \label{fig:RD_dis}
% \end{figure}
% \begin{figure}[htbp]
% \centering
%   \includegraphics[height=5.5cm, width=7.5cm]{Rate_dis_Gaussian.pdf}
% \caption {Distortion Rate curve for jointly Gaussian distribution of $(X,\theta)\sim\mathcal{N}(0,\Sigma)$, where $\Sigma$ selected randomly.}
% \label{fig:RD_Gaus}
% \end{figure}
%Observe that in the Fig.~\ref{fig:RD_dis} and Fig.~\ref{fig:RD_Gaus} the distortion value converges the bounds that we found in the Section \ref{sect:problem.statement}. [PARINAZ: Is this true? How can I see this just from looking at the plots?]
%\begin{align*}
%R(D)=I(\theta;T)\geq I(X;T)&=H(X)-H(X|T)\\
%&=H(X)-D
%\end{align*}
%where $D$ is the distortion value. The above expression shows that for each value of the distortion the rate can not be less that $H(X)-D$.\par 
%\subsection{$k$-sample Unsupervised Learning}
%To find $R^{k}_{\text{U}}(D)$, we can make use of similar analogies with the information bottleneck over the Markov chain $X - X^k - T$. 
%However, a naive implementation of the methods from \cite{tishby2000information,chechik2005information} imposes high computational and storage burdens. One can reduce those burdens by exploiting the fact that $X$ and $X^k$ are i.i.d. samples drawn from $p(x|\theta)$.
\subsubsection*{Gaussian Source}
When $X$ and $\theta$ are jointly (multivariate) Gaussian, one can appeal to the Gaussian information bottleneck, \cite{chechik2005information}, where it is shown that the optimum $T$ is a noisy linear projection of the source, which one can find iteratively or in closed form and will be described in the sequel. If $X$ is a $d$-dimensional multivariate Gaussian, however, naive application of this approach requires one to find an $dk \times dk$ projection matrix. Here again, exploitation of the structure of this problem simplifies the result.\par
Without loss of generality, let $p(x|\theta) = \mathcal{N}(\theta,\Sigma_x)$ and $p(\theta) = \mathcal{N}(0,\Sigma_\theta)$, where $\Sigma_x \in \mathbb{R}^{d \times d}$ is the covariance of the data, and $\Sigma_\theta$ is the covariance of the prior. For $k$-sample training set $X^k$ with a Gaussian source, the sample mean, $\overline{X}_k=\frac{1}{k}\sum_{i=1}^k x_i$ is a sufficient statistic for $\theta$ and we have the Markov chain $X - \theta - \overline{X}_k - T$, where $X$ is a hypothetical test point conditionaly independent of $X^k$ given $\theta$. \cite{chechik2005information} shows that the IB-optimum compression is $T = A\overline{X}_k + Z$, where $Z$ is white Gaussian noise and in our setup $A$ is a matrix whose rows are scaled left eigenvectors of the matrix
\begin{equation}
  M = \frac{\Sigma_x+\Sigma_{\theta}}{k}+\frac{k-1}{k}\Sigma_{\theta} - \Sigma_\theta (\Sigma_{x} + \Sigma_\theta)^{-1}\Sigma_\theta.
\end{equation}
Specifically, let $\lambda_1,\lambda_2,\dots$ be the ascending eigenvalues of $M_k$ and $v_1,v_2$ be the associated left eigenvectors. For $\beta>1$, only the eigenvectors $v_i$ such that $\beta_i := (1-\lambda_i)^{-1} < \beta$ are incorporated into $A$, and the resulting rate-distortion point is given parametrically by
\begin{align}
  R(\beta) &= \frac{1}{2}\sum_{i=1}^{n(\beta)} \log\left((\beta-1)\frac{1-\lambda_i}{\lambda_i} \right) \\
  D(\beta) &= \frac{1}{2}\sum_{i=1}^{n(\beta)} \log\left(\lambda_i \frac{\beta}{\beta - 1}\right) + h(X),
\end{align}
where $n(\beta)$ is the number of eigenvalues satisfying $\beta_i < \beta$. For $\beta \approx 1$, the rate is small and the distortion is close to the maximum value $h(X)$; as $\beta \to \infty$ the rate becomes large and the distortion converges to $h(X|X^k)$.

The problem setting implies structure on the compression matrix $A$ beyond what is obvious from above.
%\begin{theorem}
%  The rank of $K$ is at most $d$, and the left eigenvectors of $K$ are the left eigenvectors of the matrix $\Sigma_\theta(\Sigma_x + \Sigma_\theta)^{-1}$.
%\end{theorem}
%This result follows from the sufficiency of the sample mean $S_k$. Its implication is that, regardless of $k$, the optimum compression is a $d$-dimensional representation of the  training set $X^k$; further, one can preprocess $X^k$ to its sample mean before apply the compression. Rather than finding a $dk$-dimensional operator in general, in this case one can derive the optimum operator from the $d$-dimensional matrix $\Sigma_\theta(\Sigma_x + \Sigma_\theta)^{-1}$ and the computation of the $d$ eigenvalues of $K$.
%\setlength\belowcaptionskip{-2ex}
\subsubsection{Algorithm}
\subsubsection*{Discrete Source}
Again, for $k$-sample with a discrete source, when $X$ and $X^k$ are i.i.d. samples drawn from $p(x|\theta)$, the histogram $H_k$ of $X^k$ is a sufficient statistic for $\theta$, and we compute $p(x^k)$, $p(x|X^k)$ and $p(x,x^k)$ in terms of the histogram. Then, the iterative IB algorithm proposed in \cite{tishby2000information}, can be rewritten
%For discrete $X$, the iterative IB algorithm proposed in \cite{tishby2000information} has the following iterations applied to the Markov chain $X-X^k-T$:
\begin{align}
  q^{(n)}(t|H_k) &= \frac{q^{(n)}(t)}{Z^{(n)}(H_k,\beta)}\exp\left[-\beta D_{KL}\left[p(x|H_k)||p(x|t)\right]\right]\\
  q^{(n+1)}(t) &= \sum_{\theta}q^{(n)}(t|H_k)p(H_k)\\
  q^{(n+1)}(x|t) &= \frac{1}{q^{(n)}(t)}\sum_{\theta}q^{(n)}(t|H_k)p(H_k,x),
\end{align} 
%\begin{align*}
%  q^{(n)}(t|x^k) &= \frac{q^{(n)}(t)}{Z^{(n)}(x^k,\beta)}\exp\left[-\beta D_{KL}\left[p(x|x^k)||p(x|t)\right]\right]\\
%  q^{(n+1)}(t) &= \sum_{\theta}q^{(n)}(t|x^k)p(x^k)\\
%  q^{(n+1)}(x|t) &= \frac{1}{q^{(n)}(t)}\sum_{\theta}q^{(n)}(t|x^k)p(x^k,x),
%\end{align*} 
where $n$ is the iteration index, $q^{(n)}(t|x^k)$ is the choice for $p(t|x^k)$ at iteration $n$, and the other iterated distributions $q^{(n)}(t),q^{(n)}(x|t)$ are intermediate distributions. The number of terms in the distribution $q^{(n)}(t|x^k)$ is upper bounded to $|\mathcal{T}|k^{|\mathcal{X}|-1}$ entries by using the histogram of $X^k$. This distribution must be updated every iteration, and computing the distributions $q^{(n+1)}(t)$ and $q^{(n+1)}(x|t)$ requires summing over $q^{(n)}(t|x^k)$, $p(x^n)$, and $p(x^k,x)$, the latter two of which are computed based on the histogram and have at most $|\mathcal{T}|\cdot k^{|\mathcal{X}| - 1}$, $k^{|\mathcal{X} - 1|}$ entries, respectively. Standard cardinality bounds would suggest that $|\mathcal{T}| = \min\{|\Theta| , k^{|\mathcal{X}| - 1}\}$ is sufficient to achieve $R^{k}_{\text{B}}(D)$. This bound on $\mathcal{T}$ is established along with a fact that $T$ depends on $X^k$ only through $\theta$. 
%\begin{prop}
%  For $k$-sample unsupervised learning with a discrete source, $|\mathcal{T}| = \min\{|\Theta| , k^{|\mathcal{X}| - 1}\} + 1$ is sufficient to achieve $R^{k}_{\text{B}}(D)$. Furthermore, $q^{(n)}(t|x^k)$, $p(x^k)$, and $p(x^k,x)$ can be represented by no more than $|\mathcal{T}|\cdot k^{|\mathcal{X} - 1|}$, $k^{|\mathcal{X} - 1|}$, and $|\mathcal{X}| \cdot k^{|\mathcal{X} - 1|}$ terms, respectively.
%\end{prop}
%\begin{IEEEproof}[Proof sketch]
% Because the training points are drawn i.i.d., the distributions involving $X^k$ are invariant to permutations. Consequently, one can express the distributions in terms of the {\em histogram} of $X^k$; the histogram of $X^k$ is a sufficient statistic for $p(x|X^k)$, which bounds the number of terms in the distribution. This fact also, along with the fact that $T$ depends on $X^k$ only through $\theta$, establishes the bound on $|\mathcal{T}|$.
%\end{IEEEproof}
As a result, the problem structure allows one to reduce the complexity of the IB algorithm from exponential to polynomial when $|\mathcal{X}|$ is constant, albeit of a potentially large degree.
%\setlength\belowcaptionskip{-4ex}
\begin{figure}[H]
\centering
  \includegraphics[width=7cm]{IB_Discrete.pdf}
\caption {Rate-distortion curve for Bernoulli distribution with uniform prior and $k\in\{4,10,20,50\}$.}
\label{fig:Rate-Discrete}
\end{figure}
In Figure~\ref{fig:Rate-Discrete} we plot the rate-distortion curve for a Bernoulli distribution with a uniform prior and $|\mathcal{T}|=k+1$ is sufficient for the Bernoulli distribution. As the number of samples increase we see that the cross entropy loss decreases; however, the cross entropy loss for each sample is bounded by $H(X|X^k)$.
\subsubsection*{Gaussian Source}
For $k$-sample $X^k$ with the Gaussian distribution, the sample mean $\overline{X}_k$ is the sufficeint statistic for $\theta$, and the Markov chain is $X - \theta - \overline{X}_k - T$. \cite{chechik2005information} propose an iterative algorithm to compute the compressed representation $T^{(n)}=A^{(n)}\overline{X}_k+Z^{(n)}$, where the projection matrix $A^{(n)}$ and covariance of noise $Z^{(n)}\sim \mathcal{N}(0,\Sigma_Z^{(n)})$ is computed as:
\begin{align}
&\Sigma_Z^{(n+1)} = (\beta\Sigma_{t^{(n)}|x}-(\beta-1)\Sigma_{t^{(n)}})^{-1}\\
&A^{(n+1)}=\beta\Sigma_Z^{(n)}\Sigma_{t^{(n)}|x}^{-1}A^{(n)}(I-\Sigma_{x|\overline{X}_k}\Sigma_{\overline{X}_k}^{-1}),
\end{align}
where $\Sigma_{t^{(n)}|x}$ and $\Sigma_{t^{(n)}}$ are covariance matrix which is computed based on $T^{(n)}$ in each iteration.
\begin{figure}[H]
\centering
  \includegraphics[width=7cm]{GIB_DifferentNumebrofSamples.pdf}
\caption {Rate-distortion curve for jointly Gaussian distribution with $d=6$ and $k\in\{5,20,100,200,500\}$.}
\label{fig:Rate-Dist}
\end{figure}
%%%%%%
% \begin{theorem}
% The eigenvector of the $ \Sigma_{x^kx}\Sigma_x^{-1}\Sigma_{xx^k}\Sigma_{x^k}^{-1}$ is the combination of the eigenvector of the $\Sigma Q$.
% \end{theorem}
% \begin{proof}
% As it is represented in the (\ref{Rate}) and (\ref{bottleneck}) the GIB is function of $\beta$ and $\lambda$. Therefore, the eigenvalues of the $\Sigma_{x^k|x}\Sigma_{x^n}^{-1}$ is important for us. Based on the (\ref{x^n}), $\Sigma_{x^n|x}\Sigma_{x^n}^{-1}$ can be written as:
% \begin{align*}
% &\Sigma_{x^k|x}\Sigma_{x^n}^{-1}=I-\Sigma_{x^kx}\Sigma_x^{-1}\Sigma_{xx^k}\Sigma_{x^n}^{-1}\\
% &\Sigma_{xx^k}=\begin{bmatrix}
%     \Sigma_{\theta} & \Sigma_{\theta}  & \dots & \Sigma_{\theta} 
% \end{bmatrix}
% \end{align*}
% Therefore, by assuming $Q=(\Sigma_x+\Sigma_{\theta})^{-1}$ and $\Sigma=\Sigma_{\theta}$ we can rewrite the $\Sigma_{x^nx}\Sigma_x^{-1}\Sigma_{xx^n}\Sigma_{x^n}^{-1}$ as
% \begin{equation}
% \begin{bmatrix}
%     \Sigma Q\Sigma       & \Sigma Q\Sigma  & \dots & \Sigma Q\Sigma \\
%     \Sigma Q\Sigma       & \Sigma Q\Sigma  & \dots & \Sigma Q\Sigma \\
%     \hdotsfor{4} \\
%     \Sigma Q\Sigma       & \Sigma Q\Sigma  & \dots & \Sigma Q\Sigma
% \end{bmatrix}
% \times 
% \Sigma_{x^n}^{-1}
% \end{equation}
% Then,
% \begin{align*}
% &\Sigma_{x^k}=\begin{bmatrix}
%     U       & V^T  \\
%     V       & Q^{-1}  \\
% \end{bmatrix}, \\ 
% &\Sigma_{x^k}^{-1}=\begin{bmatrix}
%   (U-V^TQV)^{-1}   & -U^{-1}V^T(Q^{-1}-VV^T)  \\
%    -U^{-1}V^T(Q^{-1}-VV^T)  & (Q^{-1}-V^TQV)^{-1}  \\
% \end{bmatrix}\\
% &(U-V^TQV)^{-1}=(I+\sum_{i=1}^\infty(UV^TQV)^i)U^{-1} 
% \end{align*}
% where $U$ is the combination of $Q$ and $\Sigma$. Moreover, $V=\Sigma\times 1_{n\times 1}$.
% \end{proof}
% Based on our experimental results, the maximum number of the eigenvalues that we use for computing the GIB curve $n_\beta$ is the same for constant $Rate$ with different $k$ (number of samples).\par
In Figure~\ref{fig:Rate-Dist} we plot the rate-distortion curve for a Gaussian source, where $d=6$ and the covariances are drawn elementwise at random from the standard normal distribution and symmetrized. The curve is smooth because the Gaussian information bottleneck provides an exactly optimum solution.
% \begin{align*}
% h(x|x^k)-h(x|\theta)=D_{KL}\left(p(x|x^k)||p(x|t)\right)
% \end{align*}
% Fig.~\ref{fig:Rate-Sample} illustrate that by choosing the rate function as a polynomial $\log(k)$, where $k$ is the number of samples, difference between the distortion function $h(x|t)$ and $h(x|\theta)$ falls down with $1\mathbin{/}k$.
% Note that the KL-Divergence also falls down with $1\mathbin{/}k$. In conclusion, as the number of samples increases this difference $D-h(x|\theta)$ and KL-Divergence converges to each other. \par
% \begin{figure}[htbp]
% \centering
%   \includegraphics[height=5.5cm, width=7.5cm]{Rate_Samples.pdf}
% \caption {Relation between rate function and number of samples.}
% \label{fig:Rate-Sample}
% \end{figure}
% \begin{prop}\label{prpp:cardinality} Based on the Caratheodory theorem in n-letter prediction problem, $|\mathcal{T}|\leq |\mathcal{X}^k|+1$. This upper bound is linearly increase by the number of samples; however, for the discrete value of $\theta$ we can find a tighter cardinality bound.
% \begin{align}
% &R(D)=I(T;X^k)\geq I(T;\theta)\nonumber\\
% &|\mathcal{T}|\leq |\mathcal{\theta}|+1
% \end{align}
%  \end{prop} 

%  \subsection{Experimental Results}
%  In this part, we study empirically the distortion-rate curve of prediction for binary Restricted Boltzmann Machines (RBMs). First, consider the setting shown in Fig.~\ref{fig:Deep_RBM} with two neurons in the visible and hidden layers with one hidden layer. Similar to how IB method used in the discrete distribution to obtain the distortion-rate curve, we use the IB method for (RBMs). In the Fig.~\ref{fig:Dis_RBM}, we assume this structure, $X \mbox{–} \theta \mbox{–} T$, where $\theta$ is the parameters of the RBMs consists of weights and biases between visible and hidden layers, and they are selected from $\mathcal{N}(0,1)$. Two different discrete values for $\theta$ are considered in this scenario. As it is shown in Fig.~\ref{fig:Dis_RBM} the distortion $H(X|T)$ is decrease by increasing the rate $I(T;\theta)$. \\    
% \begin{figure}[htbp]
% \centering
%   \includegraphics[height=5.5cm, width=7.5cm]{IB_dis_RBM.pdf}
% \caption {Distortion-rate curve for different values of $\theta$.}
% \label{fig:Dis_RBM}
% \end{figure}    
% Now consider the continuous $\theta$ and this structure $X\mbox{-}\theta\mbox{-}X^n\mbox{–}T$, based on the \cite{Sankar privacy} and the Caratheodory theorem cardinality of the $T$ is bounded by $|\mathcal{X}_k|+1$. However, based on our experimental results even by choosing smaller cardinality for $T$ we can reach to the specific value for rate and distortion. We show the distortion-rate curve for this scenario and $|\mathcal{T}|=|\mathcal{X}_k|$, in Fig.~\ref{fig:Cos_RBM_xk}, for $|\mathcal{T}|=|\mathcal{X}|$, where  we see the distortion increases for a fix value of rate. 
% \begin{figure}[htbp]
% \centering
%   \includegraphics[height=5.5cm, width=7.5cm]{IB_con_RBM_Xk.pdf}
% \caption {Distortion-Rate curve for continuous $\theta$.}
% \label{fig:Cos_RBM_xk}
% \end{figure}
% \begin{figure}[htbp]
% \centering
%   \includegraphics[height=5.5cm, width=7.5cm]{IB_con_RBM_X.pdf}
% \caption {Distortion-Rate curve for continuous $\theta$.}
% \label{fig:Cos_RBM_x}
% \end{figure}
\subsection{Streaming Data}
%\label{sect:streaming.dataset}
%\begin{document}
%\title{Information Bottleneck Methods for Streaming data Transmission} 
%\maketitle
%In this report, we consider two main solutions for the streaming data set (as it is shown in Fig~\ref{fig:stream_model}), comprehensive and greedy solutions.
%There are two approaches to solve the streaming problem: the  {\em comprehensive solution}, where a global problem is design for all $k$ samples by considering causality, and {\em online solution}, in which data arrives one-by-one and the optimum compression $T_k$ is found for each round.
There are three approaches to solve the streaming problem: the  {\em comprehensive solution}, where we pose a global problem, and we find the global optimum solution by considering causality for a block data with a known length which is encoded sequentially. {\em online solution} for a stream data that comes one by one, in which the optimum compression $T_k$ is found for each round and we consider that the compression of other rounds $T^{-k}$ is constant. Finally, {\em two-pass solution}, where  we add the return path to the online solution to improve the results; in this setup similar to the comprehensive solution, we know the length of the block data and we want to process this data one by one. In the following part, we study {\em fundamental limits} and {\em algorithmic method} for all these three solutions.  
%\setlength\belowcaptionskip{-2ex}
%\begin{figure}[H]
%\centering
%  \includegraphics[width=5cm]{Streaming.pdf}
%\caption {Streaming data transmission model.}
%\label{fig:stream_model}
%\end{figure}
\subsubsection{Fundamental Limits}
\subsubsection*{Comprehensive Solution}
Let's assume $(X,\theta)$ are jointly Gaussian and we observe a set of $k$ i.i.d. samples $X^k = (X_1,X_2,...,X_k)$ and $X$ is a hypothetical test point conditionally
independent of $X^k$ given $\theta$ (Figure \ref{fig:stream_model}). In streaming data similar to the batch data, sample mean $\overline{X}_k=\frac{1}{k}\sum_{i=1}^k x_i$ is a sufficient statistic for $\theta$ and the Markov chain is $X-\theta-\overline{X}_k-T^k$.
Then, the computation of $D^k_\text{SC}(R)$ is equivalent to the solution of the this problem
%Then, to find $R^k_\text{S}(D)$, we use the results of the information bottleneck in \cite{{chechik2005information} for the Gaussian distribution over the Markov chain 
%and optimum $p(t_k|x_k)$ in the streaming dataset over the Markov chain $X-\theta-X^k-T_k$, we rewrite the rate-distortion problem as follows: 
%\begin{align*}
\begin{equation}\label{eq:loss_com}
\begin{split}
\max_{{p(t_1|x^1),\dots,p(t_l|x^l)}}\!\!\!\!\!\!\!\!\!\!\!\mathcal{L} = &\sum_{l=1}^k I(X;T^l)-\alpha_l I(S_l;T_l|T^{-l})
\end{split}
\end{equation}
%\end{align*}
where $I(T^l;X)=h(X)-h(X|T^l)$ determines the average distortion of all rounds and $I(S_l;T_l|T^{-l})$ determines the rate in each round, $\alpha_l$ determines the trade-off between the average distortion and rate of each round, and as it is shown in \cite{chechik2005information} $T_l$ is a noisy linear projection of the source. The comprehensive solution finds the optimum compression for each round by solving the global problem since this problem is not a convex problem, finding a closed-form solution is highly unlikely. In addition, finding the numerical solution for a Gaussian distribution and even a discrete distribution is computationally expensive as dimension of data $d$ and number of samples $k$ get big, because we need to compute $k(d\times d)$ elements of projection matrix $A$ for $k$ samples that maximize the (\ref{eq:loss_com}). 
%where $I(T^k;X)=h(X)-h(X|T^k)$ determines the average distortion of all rounds for $i\in\{1,\dots,k\}$, $I(S_i;T_i)$ determines the rate in each round, $\alpha_i$ determines the trade-off between the average distortion and rate of each round, and as it is shown in \cite{chechik2005information} $T_k$ is a noisy linear projection of the source. Although the comprehensive solution yields the optimum solution, finding a closed-form solution for a Gaussian distribution and even a discrete distribution with $k \geq 3$ is highly unlikely, since it finds the optimum solution for all encoders by solving the global problem. As a result, we design the sequential problem which leads directly to the close form solution and the iterative algorithm in the next part.   
\subsubsection*{Online Solution} 
In the online solution for stream data, computation of the $D_{SO}^k(R)$ equivalent to a conditional information bottleneck, which solves the problem
\begin{equation}
\min_{A_k}\mathcal{L}=I(\overline{X}_k;T_k|T^{-k})-\beta I(X;T_k|T^{-k}),\label{online_loss}
\end{equation}
%Since the comprehensive method cannot find a closed-form solution, we use the online approach to have a closed-form solution for a $d$-dimensional multivariate Gaussian distribution. Similar to the batch dataset, based on \cite{chechik2005information} the IB-optimum compression for each round is $T_k = AS_k + Z$, where $Z$ is the white noise with $\Sigma_Z=I_d$, $A$ is the projection matrix, and $S_k$ is a sufficient statistic for $\theta$. Then, the rate-distortion problem can be written as
%In this section, for the Gaussian variables, we use the greedy approach 
%\begin{align*}
%\min_{A}\mathcal{L}&=I(T_k;S_k|T_{-k})-\beta I(X;T_k|T_{-k})\\ &=(1-\beta)h(T_k|T_{-k})-h(T_k|S_k)+\beta h(T_k|T_{-k},X)\\
% &=\!(1\!-\!\beta)\log(\Sigma_{T_k|T_{-k}}\!)\!-\!\log(\Sigma_Z)\!+\!\beta\log(\Sigma_{T_k|X,T_{-k}}\!)\\
% &=\!(1\!-\!\beta)\!\log(A\!\Sigma_{S_k|T_{-k}}\!A^T\!\!+\!\!I_d)\!+\!\!\beta\log(\!A\Sigma_{S_k\!|\!X,T_{-k}}A^T\!\!+\!\!I_d\!),
% \end{align*}
%where $T_{-k}=(T_1,T_2,\dots,T_{k-1})$. Taking the derivative of this loss function with respect to the projection matrix $A_k$, we find that $A$ is the matrix whose rows are scaled left eigenvalues of the matrix
where $T^{-k}:=\{T_1,T_2,\dots,T_{k-1}\}$. In this setup $\beta$ shows the trade-off between rate and relevant information and for $\beta \approx 1$, the rate of each round $I(T_k;\overline{X}_k|T^{-k})$ is small and the distortion $H(X|T^k)$ is close to $H(X|T^{-k})$, when $\beta \to \infty$ the rate becomes large and the distortion converges to $H(X|\overline{X}_k)$. In the following theorem, we characterize the optimum $A_k$:
\begin{theorem}\label{theorem:1}
The optimum projection $A_k$ that solves (\ref{online_loss}) for some $\beta$ satisfies
  \begin{equation}\label{projection}
    A_k=
    \begin{cases}
      [0,\dots,0] & 0<\beta<\beta_{c_1} \\
      [\alpha_1v_1^T,0,\dots] & \beta_{c_1}<\beta<\beta_{c_2}\\
             .            \\
             .            \\
             .            \\
      [\alpha_1v_1^T,\dots,\alpha_kv_k^T] & \beta_{c_{k-1}}<\beta<\beta_{c_{k}}
    \end{cases},
  \end{equation}
where $\lambda_1,\lambda_2, . . .$ are the ascending eigenvalues of
$M = \Sigma_{\overline{X}_k|T^{-k},X}\Sigma^{-1}_{\overline{X}_k|T^{-k}}$, $v_1, v_2, \dots$ are the associated left eigenvectors, and $\beta_{c}=\frac{1}{1-\lambda_i}$ are critical values for $\beta$ and $\alpha_i=\sqrt{\frac{\beta(1-\lambda_i)-1}{\lambda_i(v_i^T\Sigma_{\overline{X}_k|T^{-k}}v_i)}}$.
\end{theorem}
\begin{proof}
We first rewrite the loss function in terms of the entropies
\begin{align*}
\min_{A_k}\mathcal{L}&=I(\overline{X}_k;T_k|T^{-k})-\beta I(X;T_k|T^{-k})\\ &=(1-\beta)h(T_k|T^{-k})-h(T_k|\overline{X}_k)+\beta h(T_k|T^{-k},X)\\
 &=\!(1\!-\!\beta)\log(\Sigma_{T_k|T^{-k}}\!)\!-\!\log(\Sigma_Z)\!+\!\beta\log(\Sigma_{T_k|X,T^{-k}}\!)\\
 &=\!(1\!-\!\beta)\!\log(A_k\!\Sigma_{\overline{X}_k|T^{-k}}\!A_k^T\!\!+\!\!I_d)\\
 &+\beta\log(\!A_k\Sigma_{\overline{X}_k\!|\!X,T^{-k}}A_k^T\!\!+\!\!I_d\!),
 \end{align*}
By taking derivative of the loss function with respect to the $A$
\begin{align*}
\frac{\delta\mathcal{L}}{\delta A_k}&=(1-\beta)(A_k\Sigma_{\overline{X}_k|T^{-k}}A_k^T+I_d)^{-1}2A_k\Sigma_{\overline{X}_k|T^{-k}}\\ &+ \beta(A_k\Sigma_{\overline{X}_k|X,T^{-k}}A_k^T+I_d)^{-1}2A_k\Sigma_{\overline{X}_k|X,T^{-k}}
\end{align*} 
In order to obtain minimum of the loss function $\mathcal{L}$, we equal $\frac{\delta\mathcal{L}}{\delta A_k}=0$ and we have:
\begin{align}\label{eq:eigeneqution}
&\frac{\beta-1}{\beta}\left[(A_k\Sigma_{\overline{X}_k|T^{-k},X}A_k^T+I_d)(A_k\Sigma_{\overline{X}_k|T^{-k}}A_k^T+I_d)^{-1}\right]A_k\\\nonumber
&=A_k\left[\Sigma_{\overline{X}_k|X,T^{-k}}\Sigma_{\overline{X}_k|T^{-k}}^{-1}\right]
\end{align}
This equation is an eigenvalue problem and $A$ is the eigenvector of $\Sigma_{\overline{X}_k|X,T^{-k}}\Sigma_{\overline{X}_k|T^{-k}}^{-1}$. Then, we can substitute $A_k=UV$ and $V\Sigma_{\overline{X}_k|X,T^{-k}}\Sigma_{\overline{X}_k|T^{-k}}^{-1}=LV$ similar to \cite{chechik2005information} and rewrite the (\ref{eq:eigeneqution}):
\begin{align*}
&\frac{\beta\!-\!1}{\beta}\left[(U\Sigma_{\overline{X}_k|T^{-k},X}U^T+I_d)(U\Sigma_{\overline{X}_k|T^{-k}}U^T+I_d)^{-1})\right]U\\
&=UL
\end{align*}
Considering $\Sigma_{\overline{X}_k|T^{-k}}=V^{-1}SV$ and $\Sigma_{\overline{X}_k|T^{-k},X}=V^{-1}SLV$ and multiplying by $U^{-1}$ from left and $U^{-1}(U\Sigma_{\overline{X}_k|T^{-k}}U^T+I_d)^{-1}$ by right we will have:
\begin{align}\label{eqn:Ucomputation}
UU^T=\left[\beta(I-L)-I\right](LS)^{-1}
\end{align}
Therefore, $A_k=UV$ in which $V$ is the eigenvector of the $\Sigma_{\overline{X}_k|T^{-k},X}\Sigma_{\overline{X}_k|T^{-k}}$ and $U$ is computed based on (\ref{eqn:Ucomputation}). 
\end{proof}
\subsubsection*{Two-pass Online Solution}
To improve the result of the online solution and make the results closer to the optimum solution, we introduce the two-pass version of the online solution that solves the problem from $(k-1)$-th round to the first round by solving the following loss function 
\begin{align}\label{eq:recursive online}
\min_{A_{k-1}}\!\mathcal{L}\!=\!I(\overline{X}\!_{k-1};T\!_{k-1}\!|T^{-(k-1)}\!,T_k)\!-\!\beta I(X;T\!_{k-1}|T^{-(k-1)},T_k)
\end{align} 
where $T^{-(k-1)}=\{T_1,T_2,\dots,T_{k-2}\}$. In this setup, similar to the online solution, $\beta$ shows the trade-off between rate and relevant information and for $\beta \approx 1$, the rate of each round $I(\overline{X}_{k-1};T_{k-1}|T^{-(k-1)})$ is small and the distortion $H(X|T^k)$ is close to $H(X|T^{-(k-1)},T_k)$, when $\beta \to \infty$ the rate becomes large and the distortion converges to $H(X|\overline{X}_k)$. Similar to the theorem \ref{theorem:1}, we characterize the optimum projection matrix from $(k-1)$-round to the previous round ($(k-2)$-th round) in the following theorem:
\begin{theorem}\label{theorem2}
The optimum projection matrix $A_{k-1}$ that solves (\ref{eq:recursive online}) 
   \begin{equation}
    A_{k-1}=
    \begin{cases}
      [0,\dots,0] & 0<\beta<\beta_{c_1} \\
      [\alpha_1v_1^T,0,\dots] & \beta_{c_1}<\beta<\beta_{c_2}\\
             .            \\
             .            \\
             .            \\
      [\alpha_1v_1^T,\dots,\alpha_kv_k^T] & \beta_{c_{k-1}}<\beta<\beta_{c_{k}}
    \end{cases},
  \end{equation}
where $\lambda_1,\lambda_2, . . .$ are the ascending eigenvalues of
$K = \Sigma_{\overline{X}_k|T^{-k},X}\Sigma^{-1}_{\overline{X}_k|T^{-k}}$, $v_1, v_2, \dots$ are the associated left eigenvectors, and $\beta_{c}=\frac{1}{1-\lambda_i}$ are critical values for $\beta$ and $\alpha_i=\sqrt{\frac{\beta(1-\lambda_i)-1}{\lambda_i(v_i^T\Sigma_{\overline{X}_k|T^{-k}}v_i)}}$.
\begin{proof}
The proof is similar to theorem \ref{theorem:1} and to avoid repetition we do not write the proof. 
\end{proof}
\end{theorem}
\subsubsection{Algorithm}
\subsubsection*{Comprehensive Solution}
Comprehensive solution finds the optimum solution for a block data with a known length which is encoded sequentially by considering causality. Since we can not find a closed-form solution in the comprehensive case, we solve this optimization problem for $k=2$ using numerical optimization methods for scalar case. Figure \ref{fig:Compare_Stream} demonstrates the total distortion ($H(X|T_1)+H(X|T^2)$) versus the total rate ($I(\overline{X}_1;T_1)+I(\overline{X}_2;T^2|T_1)$), rate-distortion curve, for both comprehensive and online solutions. Although the comprehensive solution converges to the smaller distortion for the same rate, the result of comprehensive solution is scattered since we use the numerical optimization methods (fminunc function in Matlab) to solve (\ref{eq:loss_com}) and in some area this function finds the local minimum. Therefore, we plot the convex hull of the solution since we know the rate-distortion curve is convex.  
%that the comprehensive solution is the optimum solution and converges to the GIB solution, in which we use the all rate in the last round, while the online solution is strictly sub-optimum. \par
 \begin{figure}[htb]
\centering
  \includegraphics[width=7cm]{CompareStream.pdf}
\caption {Comparison between online and comprehensive solutions by rate-distortion curve, where $K=2$ and "x" axis is the total rates and "y" axis is the total distortion. }
\label{fig:Compare_Stream}
\end{figure}
\subsubsection*{Online Solution} Theorem \ref{theorem:1} states that the optimal projection matrix of each round in the online solution consists of eigenvalues of $M$, in order to compute the whole projection matrix $A$ for the stream dataset $X^k$ we propose an iterative algorithm as follows: 
%\begin{equation*}
% K = \Sigma_{S_k|T_{-k},X}\Sigma^{-1}_{S_k|T_{-k}}.
%\end{equation*}
%Therefore, as it is satated in \cite{chechik2005information}, the projection matrix $A$ in each round is computed as
%  \begin{equation*}
%    A_k=
%    \begin{cases}
%      [0,\dots,0] & 0<\beta<\beta_{c_1} \\
%      [\alpha_1v_1^T,0,\dots] & \beta_{c_1}<\beta<\beta_{c_2}\\
%             .            \\
%             .            \\
%             .            \\
%    \end{cases}.
%  \end{equation*}
%where $\lambda_1,\lambda_2, . . .$ are the ascending eigenvalues of
%$K$, $v_1, v_2, \dots$ are the associated left eigenvectors, and $\beta_{c}=\frac{1}{1-\lambda_i}$ are critical values for $\beta$ and $\alpha_i=\sqrt{\frac{\beta(1-\lambda_i)-1}{\lambda_i(v_i^T\Sigma_{S_k|T_{-k}}v_i)}}$.   
%%Let $\lambda_1,\lambda_2, . . .$ be the ascending eigenvalues of
%%$K$ and $v_1, v_2, \dots$ be the associated left eigenvectors.
%Based on the \cite{chechik2005information}, we can compute the rate and average distortion for each round as follows: 
%\begin{align*}
%  &R(\beta) = \frac{1}{2}\sum_{i=1}^{n(\beta)} \log\left((\beta-1)\frac{1-\lambda_i}{\lambda_i} \right) \\
%  &I(X;T_k|T_{-k})_{\beta} = \frac{1}{2}\sum_{i=1}^{n(\beta)} \log\left(\lambda_i \frac{\beta}{\beta - 1}\right).
%\end{align*}
%Therefore, we can derive an iterative algorithm:
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[htb]
\caption{Online Solution for Streaming data}
\begin{algorithmic}[1]
\label{algorithm_1}
\STATE {Initiate the values of $\Sigma_{\theta}, \Sigma_n$ and $K$ number of rounds.}
\FOR{each round, $k=1:K$ \do }
\STATE {$\Sigma_{\overline{X}_k}\leftarrow\Sigma_n/n+\Sigma_{\theta}$.}
\STATE {$\Sigma_{T^{-k}}\leftarrow A\Sigma_{X^k}A^T+I_d$.}
\STATE {$\Sigma_C\leftarrow [(\Sigma_x\!+\!(k-1)\Sigma_{\theta})A_1,\dots,(\Sigma_x\!+\!(k-1)\Sigma_{\theta})A_k/k]$}
\STATE {$\Sigma_{\overline{X}_k|T^{-k}}\leftarrow\Sigma_{\overline{X}_k}-\Sigma_C\Sigma_{T^{-k}}^{-1}\Sigma_C^T$}
\STATE {$\Sigma_{\overline{X}_k|X,T^{-k}}\leftarrow\Sigma_{\overline{X}_k}-[\Sigma_{\theta},\Sigma_C]\Sigma_{X,T^{-k}}^{-1}[\Sigma_{\theta},\Sigma_C]^T$.}
\STATE  {Compute $M$ and eigenvalues $\lambda_1,\lambda_2,\dots$ and left eigenvectors $v_1,v_2,\dots$}
\STATE  {Compute the projection matrix of each round, $A_k$ based on \ref{projection}.}
\STATE {Compute the critical values of $\beta$ for each eigenvalue as $\beta_c=\frac{1}{1-\lambda}$, and initiate value for $\beta_{size}$.} 
%\FOR{$\beta$ = $\beta_c:\beta_{size}$ \do }
%\STATE \begin{equation}\begin{aligned}
%  &R(\beta) = \frac{1}{2}\sum_{i=1}^{n(\beta)} \log\left((\beta-1)\frac{1-\lambda_i}{\lambda_i} \right) \\
%  &I(X;T_k|T_{-k})_{\beta} = \frac{1}{2}\sum_{i=1}^{n(\beta)} \log\left(\lambda_i \frac{\beta}{\beta - 1}\right)\nonumber
%\end{aligned}
%\end{equation}
%\ENDFOR
\STATE {$A=diag(A_1,\dots,A_k)$}
\ENDFOR
\end{algorithmic}
\end{algorithm}
\noindent
where $\beta_{size}$ determines the rank of the projection matrix in each round and depends on the $\beta_c$. In this algorithm, first, for each round (from 1 to $K$) we find the matrix $M$ and its eigenvalues and eigenvectors. Then, we compute the projection matrix $A_k$ of this round according to $\beta_{size}$ and the eigenvalues and eigenvectors of the matrix $M$ and save it to calculate the $K$ for the next round.\par 
Similar to the batch data, from the sufficiency of the sample mean $\overline{X}_k$, we see that regardless of $k$, the optimum compression of each round $T_k$ is a $d$-dimensional representation of the  training set $X^k$; however, in our algorithm the global projection matrix $A$ is a $dk$-dimensional diagonal matrix operator, which we need it to compute the $\Sigma_{T^{-k.}}$. In general, in this problem one can derive the optimum operator from the $d$-dimensional matrix $M$ and compute the projection matrix $A_k$ in each round  and store it into the $A=diag(A_1,\dots,A_k)$. \par
 \begin{figure}[htb]
\centering
  \includegraphics[width=7cm]{DisSamplesDifRates.pdf}
\caption {Number of Samples-Distortion curve for jointly Gaussian distribution with $d=10$ and $R\in\{4,8,10,14,16\}$.}
\label{fig:Rate-RelStream}
\end{figure}
In Figure \ref{fig:Rate-RelStream} we show the sample-distortion curve for a jointly Gaussian distribution, where $h(X|\theta)$ and $k$ represent the distortion function and the number of rounds or the number of samples that we use, receptively. In addition, for a fixed rate, as the number of samples increase we see that the distortion decreases; however, for a sufficiently large number of samples, this reduction becomes negligible. This can be interpreted as the eigenvalue of the $M$ matrix tends to 1.
\subsubsection*{Two-pass Solution}
In theorem \ref{theorem2} we propose a two-pass method, where  we encode a block data with known length in each round in contrast to the online solution. Algorithm \ref{algorithm_2} computes the optimum projection of each round (assuming other rounds are constant) based on this chain $A_1-A_2-\dots-A_K$ and then obtains the optimum projection of each iteration according to the two-pass chain $A_K-A_{K-1}-\dots-A_1$. We summarized this procedure in Algorithm \ref{algorithm_2}. \par
\begin{algorithm}[htb]
\caption{Two-pass Algorithm}
\begin{algorithmic}[1]
\label{algorithm_2}
\STATE {Initiate the values of $\Sigma_{\theta}, \Sigma_n$, $K$ and $N$ covariance of the $\theta$ and noise, number of rounds and number of iteration that we need to run the two-pass algorithm, respectively.}
\FOR{each round, $n=1:N$ \do }
\FOR{each round, $k=1:K$ \do }
\STATE {$\Sigma_{\overline{X}_k}\leftarrow\Sigma_n/n+\Sigma_{\theta}$.}
\STATE {$\Sigma_{T^{-k}}\leftarrow A\Sigma_{X^k}A^T+I_d$.}
\STATE {$\Sigma_C\leftarrow [(\Sigma_x\!+\!(k-1)\Sigma_{\theta})A_1,\dots,(\Sigma_x\!+\!(k-1)\Sigma_{\theta})A_k/k]$}
\STATE {$\Sigma_{\overline{X}_k|T^{-k}}\leftarrow\Sigma_{\overline{X}_k}-\Sigma_C\Sigma_{T^{-k}}^{-1}\Sigma_C^T$}
\STATE {$\Sigma_{\overline{X}_k|X,T^{-k}}\leftarrow\Sigma_{\overline{X}_k}-[\Sigma_{\theta},\Sigma_C]\Sigma_{X,T^{-k}}^{-1}[\Sigma_{\theta},\Sigma_C]^T$.}
\STATE  {Compute the projection matrix of each round, $A_i$ based on \ref{projection}.}
\STATE {$A=diag(A_1,\dots,A_k)$}
\ENDFOR
\FOR{$k=K-1:1$ \do }
%\STATE {$\Sigma_{\overline{X}_k}\leftarrow\Sigma_n/n+\Sigma_{\theta}$.}
\STATE {$\Sigma_{T^{-k}}\leftarrow$ eliminate $k$-th row and column of the $\Sigma_{T^K}$.}
%\STATE {$\Sigma_C\leftarrow [(\Sigma_x\!+\!(k-1)\Sigma_{\theta})A_1,\dots,(\Sigma_x\!+\!(k-1)\Sigma_{\theta})A_k/k]$}
\STATE {$\Sigma_{\overline{X}_k|T^{-k}}\leftarrow\Sigma_{\overline{X}_k}-\Sigma_C\Sigma_{T^{-k}}^{-1}\Sigma_C^T$}
\STATE {$\Sigma_{\overline{X}_k|X,T^{-k}}\leftarrow\Sigma_{\overline{X}_k}-[\Sigma_{\theta},\Sigma_C]\Sigma_{X,T^{-k}}^{-1}[\Sigma_{\theta},\Sigma_C]^T$.}
%\STATE  {Compute $K$ and eigenvalues $\lambda_1,\lambda_2,\dots$ and left eigenvectors $v_1,v_2,\dots$}
\STATE  {Compute the projection matrix of each round, $A_k$ based on \ref{projection}.}
%\STATE {Compute the critical values of $\beta$ for each eigenvalue as $\beta_c=\frac{1}{1-\lambda}$, and initiate value for $\beta_{size}$.} 
\STATE {$A^{(n)}=diag(A_1,\dots,A_k)$}
\STATE {Update $\Sigma_{T^K}\leftarrow A^{(n)}\Sigma_{X^K}A^{(n)T}+I_{Kd}$}
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}
In each iteration of this algorithm, at the first part, we compute the covariance matrix $\Sigma_{T^K}$ and projection matrix $A$. In the second part of the algorithm, we compute $\Sigma_{T^{-(k)}}$ based on the $\Sigma_{T^K}$ and then compute the projection matrix of each round $A_k$ and update the whole projection matrix $A^{(n)}$, then update the $\Sigma_{T^K}$ and use it for computation of the next round of the data. At the end, we compute the projection matrix for the $n$-th iteration $A^{(n)}$.\par
We show difference between distortion and its lower bound in terms of the rate, in Figure \ref{fig:Rate-Dis-Recursive}, where we show that the two-pass algorithm after one iteration has the better performance in compare of the online algorithm. In the two-pass algorithm projection matrix $A$ converges to the optimum value rapidly, because the eigenvalues of the matrix $M$ converges to the 1 rapidly. As a result, in Figure \ref{fig:Rate-Dis-Recursive} the difference of performance between $k=4$ and $k=1$ in the two-pass algorithm is very small. The two-pass algorithm improves the results; however, based on the number of iteration that we want to run algorithm it needs more computation and time, so it is not suitable for the online communication.\par
%\setlength\belowcaptionskip{-2.5ex}
 \begin{figure}[htb]
\centering
  \includegraphics[width=7cm]{DisRatesRcrVsOnline.pdf}
\caption {Rate-Distortion curve for jointly Gaussian distribution with $d=10$ and $k=\{1,4\}$ for the online algorithm and $k=\{1,4\}$ for two-pass algorithm after one iteration.}
\label{fig:Rate-Dis-Recursive}
\end{figure}
The rate-distortion curve, illustrated in figure \ref{fig:Rate-Dis-Com-Rcr}, compares the comprehensive and two-path solutions, in which comprehensive solution is the optimum solution by considering causality. However, figure \ref{fig:Rate-Dis-Com-Rcr} shows that two-path solution out performs since in this solution, the first pass only considers the previous choices for the projection matrix $A=diag(A_1,\dots,A_k)$, whereas in the second pass we optimize each $A_k$ given all of the other projection matrices.\par
 \begin{figure}[htb]
\centering
  \includegraphics[width=7cm]{CompareRcrComprehensive.pdf}
\caption {Rate-distortion curve for both comprehensive and two-path solutions, where $K=2$ and "x" axis is the total rates and "y" axis is the total distortion. .}
\label{fig:Rate-Dis-Com-Rcr}
\end{figure} 
Finally, we show the dependency of the rate on the number of samples $k$ for Gaussian sources. For the Gaussian sources, as $k \to \infty$ the gap between the distortion $H(X|X^k)$ given direct access to the training set and the best case distortion $H(X|\theta)$ goes to zero; equivalently, the mutual information gap $I(X;\theta) - I(X;X^k)$ goes to zero. Figure \ref{fig:Rate-sample} shows the gap between $h(X|T)$ and $h(X|X^k)$ for different rate functions. As it demonstrate for $R = \Omega(\log(k))$ the gap between $h(X|T)$ and $h(X|X^k)$ goes to zero after 6 samples, also this function for rate has the optimum decay of the gap between $h(X|T)$ and $h(X|\theta)$ among other functions for rate.
%\setlength\belowcaptionskip{-1.5ex}
\begin{figure}[htb]
\centering
  \includegraphics[width=7cm]{Rate_Samples.pdf}
\caption {Number of Samples-distortion curve for different rate functions against the $h(X|X^k)$ and $h(X|\theta)$.}
\label{fig:Rate-sample}
\end{figure}
%\begin{thebibliography}{9}
%\bibitem{GIB}
%Chechik, G. A. (2005). Information bottleneck for Gaussian variables. Journal of Machine Learning Research 6, 165-188.
%\end{thebibliography}
%\end{document}
%for every $\overline{X}_k$ and $T_k$  with jointly Gaussian distribution, we can represent the linear transformation 

 %In addition, the Markov chain is now $X-\theta-S_k-T_k$. 
%As reference \cite{chechik2005information}shows that the IB-optimum compression is $T_k = AS_k + Z$, where $Z$ is white Gaussian noise and $A$ is a matrix whose rows are scaled left eigenvectors of the matrix

==> scaling.tex <==
%!TEX root = main.tex
\section{Scaling of Compression Rate with $k$}\label{sect:scaling}
Finally, we discuss the dependency of the rate on the number of samples $k$ for continuous sources. For unsupervised learning with continuous sources, as $k \to \infty$ the gap between the distortion $h(X|X^k)$ given direct access to the training set and the best case distortion $h(X|\theta)$ goes to zero; equivalently, the mutual information gap $I(X;\theta) - I(X;X^k)$ goes to zero. An important question is the rate needed to ensure that the gap $I(X;\theta) - I(X;T)$ goes to zero at the same rate. For sources described by smooth, continous parametric families $p(x|\theta)$, we argue that the rate should scale as $\Omega(\log(k))$ via the following argument: By the data-processing inequality and the universal capacity-redundancy result of Clarke and Barron \cite{Clarke_Barron}, $I(X;X^k) \approx \log(k)$ for smooth, continuous parametric families. Since the compression rate $I(X^k;T) \geq I(X;T)$, one needs $R = \Omega(\log(k))$ to ensure that the gap $I(X;\theta) - I(X;T)$ decays no slower than $I(X;\theta) - I(X;X^k)$. We observe in numerical experiments that $R = \Omega(\log(k))$ is also sufficient for optimum decay of the gap, but we suspect that proving sufficiency is a challenging task. A similar argument holds in the case of supervised learning.\par
Figure \ref{fig:Rate-sample} shows the gap between $h(X|T)$ and $h(X|X^k)$ for different rate functions. As it demonstrate for $R = \Omega(\log(k))$ the gap between $h(X|T)$ and $h(X|X^k)$ goes to zero after 6 samples, also this function for rate has the optimum decay of the gap between $h(X|T)$ and $h(X|\theta)$ among other functions for rate.
%\setlength\belowcaptionskip{-1.5ex}
\begin{figure}[htb]
\centering
  \includegraphics[width=7cm]{Rate_Samples.pdf}
\caption {Number of Samples-distortion curve for different rate functions against the $h(X|X^k)$ and $h(X|\theta)$.}
\label{fig:Rate-sample}
\end{figure}


==> stream.tex <==
%!TEX root = main.tex
\section{streaming data}
\label{sect:streaming.dataset}
%\begin{document}
%\title{Information Bottleneck Methods for Streaming data Transmission} 
%\maketitle
%In this report, we consider two main solutions for the streaming data set (as it is shown in Fig~\ref{fig:stream_model}), comprehensive and greedy solutions.
%There are two approaches to solve the streaming problem: the  {\em comprehensive solution}, where a global problem is design for all $k$ samples by considering causality, and {\em online solution}, in which data arrives one-by-one and the optimum compression $T_k$ is found for each round.
There are two approaches to solve the streaming problem: the  {\em comprehensive solution}, where we pose a global problem, and we find the global optimum solution by considering causality, and {\em online solution}, in which the optimum compression $T_k$ is found for each round and we consider that the compression of other rounds $T_{-k}$ is constant.
%\setlength\belowcaptionskip{-2ex}
\begin{figure}[H]
\centering
  \includegraphics[width=5cm]{Streaming.pdf}
\caption {Streaming data transmission model.}
\label{fig:stream_model}
\end{figure}
\subsubsection{Comprehensive solution}
Let's assume $(X,\theta)$ are jointly Gaussian and we observe a set of $k$ i.i.d. samples $X^k = (X_1,X_2,...,X_k)$ and $X$ is a hypothetical test point conditionally
independent of $X^k$ given $\theta$ (Figure \ref{fig:stream_model}). In streaming dataset similar to the batch dataset, sample mean $S_k=\frac{1}{k}\sum_{i=1}^k x_i$ is a sufficient statistic for $\theta$ and the Markov chain is $X-\theta-S_k-T^k$.
Then, the computation of $R^k_\text{S}(D)$ is equivalent to the solution of the this problem
%Then, to find $R^k_\text{S}(D)$, we use the results of the information bottleneck in \cite{{chechik2005information} for the Gaussian distribution over the Markov chain 
%and optimum $p(t_k|x_k)$ in the streaming dataset over the Markov chain $X-\theta-X^k-T_k$, we rewrite the rate-distortion problem as follows: 
%\begin{align*}
\begin{equation*}
\begin{split}
\min_{{p(t_1|S_1),\dots,p(t_k|S_k)}}\!\!\!\!\!\!\!\!\!\!\!\mathcal{L} = &I(T^k;X)-\alpha_1 I(S_1;T_1)\\&-\alpha_2 I(S_2;T_2) \dots 
-\alpha_k I(S_k;T_k),
\end{split}
\end{equation*}
%\end{align*}
where $I(T^k;X)=h(X)-h(X|T^k)$ determines the average distortion of all rounds for $i\in\{1,\dots,k\}$, $I(S_i;T_i)$ determines the rate in each round, $\alpha_i$ determines the trade-off between the average distortion and rate of each round, and as it is shown in \cite{chechik2005information} $T_k$ is a noisy linear projection of the source. The comprehensive solution finds the optimum compression for each round by solving the global problem since this problem is not a convex problem, finding a closed-form solution for a Gaussian distribution and even a discrete distribution with $k \geq 3$ is highly unlikely
%where $I(T^k;X)=h(X)-h(X|T^k)$ determines the average distortion of all rounds for $i\in\{1,\dots,k\}$, $I(S_i;T_i)$ determines the rate in each round, $\alpha_i$ determines the trade-off between the average distortion and rate of each round, and as it is shown in \cite{chechik2005information} $T_k$ is a noisy linear projection of the source. Although the comprehensive solution yields the optimum solution, finding a closed-form solution for a Gaussian distribution and even a discrete distribution with $k \geq 3$ is highly unlikely, since it finds the optimum solution for all encoders by solving the global problem. As a result, we design the sequential problem which leads directly to the close form solution and the iterative algorithm in the next part.   
\subsubsection{Online Solution} 
In the online solution for stream dataset, computation of the $R_s^k(D)$ equivalent to a conditional information bottleneck, which solves the problem
\begin{equation}
\min_{A_k}\mathcal{L}=I(T_k;S_k|T_{-k})-\beta I(X;T_k|T_{-k}),\label{online_loss}
\end{equation}
%Since the comprehensive method cannot find a closed-form solution, we use the online approach to have a closed-form solution for a $d$-dimensional multivariate Gaussian distribution. Similar to the batch dataset, based on \cite{chechik2005information} the IB-optimum compression for each round is $T_k = AS_k + Z$, where $Z$ is the white noise with $\Sigma_Z=I_d$, $A$ is the projection matrix, and $S_k$ is a sufficient statistic for $\theta$. Then, the rate-distortion problem can be written as
%In this section, for the Gaussian variables, we use the greedy approach 
%\begin{align*}
%\min_{A}\mathcal{L}&=I(T_k;S_k|T_{-k})-\beta I(X;T_k|T_{-k})\\ &=(1-\beta)h(T_k|T_{-k})-h(T_k|S_k)+\beta h(T_k|T_{-k},X)\\
% &=\!(1\!-\!\beta)\log(\Sigma_{T_k|T_{-k}}\!)\!-\!\log(\Sigma_Z)\!+\!\beta\log(\Sigma_{T_k|X,T_{-k}}\!)\\
% &=\!(1\!-\!\beta)\!\log(A\!\Sigma_{S_k|T_{-k}}\!A^T\!\!+\!\!I_d)\!+\!\!\beta\log(\!A\Sigma_{S_k\!|\!X,T_{-k}}A^T\!\!+\!\!I_d\!),
% \end{align*}
%where $T_{-k}=(T_1,T_2,\dots,T_{k-1})$. Taking the derivative of this loss function with respect to the projection matrix $A_k$, we find that $A$ is the matrix whose rows are scaled left eigenvalues of the matrix
where $T_{-k}=(T_1,T_2,\dots,T_{k-1})$ and in the following theorem, we characterize the optimum $A_k$.
\begin{theorem}
The optimum projection $A_k$ that solves (\ref{online_loss}) for some $\beta$ satisfies
  \begin{equation}
    A_k=
    \begin{cases}
      [0,\dots,0] & 0<\beta<\beta_{c_1} \\
      [\alpha_1v_1^T,0,\dots] & \beta_{c_1}<\beta<\beta_{c_2}\\
             .            \\
             .            \\
             .            \\
      [\alpha_1v_1^T,\dots,\alpha_kv_k^T] & \beta_{c_{k-1}}<\beta<\beta_{c_{k}}
    \end{cases}.
  \end{equation}\label{projection}
where $\lambda_1,\lambda_2, . . .$ are the ascending eigenvalues of
$K = \Sigma_{S_k|T_{-k},X}\Sigma^{-1}_{S_k|T_{-k}}$, $v_1, v_2, \dots$ are the associated left eigenvectors, and $\beta_{c}=\frac{1}{1-\lambda_i}$ are critical values for $\beta$ and $\alpha_i=\sqrt{\frac{\beta(1-\lambda_i)-1}{\lambda_i(v_i^T\Sigma_{S_k|T_{-k}}v_i)}}$.
\end{theorem}
\begin{proof}
We first rewrite the loss function in terms of the entropies
\begin{align*}
\min_{A}\mathcal{L}&=I(T_k;S_k|T_{-k})-\beta I(X;T_k|T_{-k})\\ &=(1-\beta)h(T_k|T_{-k})-h(T_k|S_k)+\beta h(T_k|T_{-k},X)\\
 &=\!(1\!-\!\beta)\log(\Sigma_{T_k|T_{-k}}\!)\!-\!\log(\Sigma_Z)\!+\!\beta\log(\Sigma_{T_k|X,T_{-k}}\!)\\
 &=\!(1\!-\!\beta)\!\log(A\!\Sigma_{S_k|T_{-k}}\!A^T\!\!+\!\!I_d)\!+\!\!\beta\log(\!A\Sigma_{S_k\!|\!X,T_{-k}}A^T\!\!+\!\!I_d\!),
 \end{align*}
By taking derivative 
\end{proof}
This theorem states that the optimal projection consists of eigenvalues of $K$, in order to compute the whole projection matrix $A$ for dataset $X_k$ we propose an iterative algorithm as follows: 
%\begin{equation*}
% K = \Sigma_{S_k|T_{-k},X}\Sigma^{-1}_{S_k|T_{-k}}.
%\end{equation*}
%Therefore, as it is satated in \cite{chechik2005information}, the projection matrix $A$ in each round is computed as
%  \begin{equation*}
%    A_k=
%    \begin{cases}
%      [0,\dots,0] & 0<\beta<\beta_{c_1} \\
%      [\alpha_1v_1^T,0,\dots] & \beta_{c_1}<\beta<\beta_{c_2}\\
%             .            \\
%             .            \\
%             .            \\
%    \end{cases}.
%  \end{equation*}
%where $\lambda_1,\lambda_2, . . .$ are the ascending eigenvalues of
%$K$, $v_1, v_2, \dots$ are the associated left eigenvectors, and $\beta_{c}=\frac{1}{1-\lambda_i}$ are critical values for $\beta$ and $\alpha_i=\sqrt{\frac{\beta(1-\lambda_i)-1}{\lambda_i(v_i^T\Sigma_{S_k|T_{-k}}v_i)}}$.   
%%Let $\lambda_1,\lambda_2, . . .$ be the ascending eigenvalues of
%%$K$ and $v_1, v_2, \dots$ be the associated left eigenvectors.
%Based on the \cite{chechik2005information}, we can compute the rate and average distortion for each round as follows: 
%\begin{align*}
%  &R(\beta) = \frac{1}{2}\sum_{i=1}^{n(\beta)} \log\left((\beta-1)\frac{1-\lambda_i}{\lambda_i} \right) \\
%  &I(X;T_k|T_{-k})_{\beta} = \frac{1}{2}\sum_{i=1}^{n(\beta)} \log\left(\lambda_i \frac{\beta}{\beta - 1}\right).
%\end{align*}
%Therefore, we can derive an iterative algorithm:
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[H]
\caption{Greedy Solution for Streaming dataset}
\begin{algorithmic}[1]
\label{algorithm_SD}
\STATE {Initiate the values of $\Sigma_{\theta}, \Sigma_n$ and $N$ number of rounds.}
\FOR{each round, $k=1:N$ \do }
\STATE {$\Sigma_{S_k}\leftarrow\Sigma_n/n+\Sigma_{\theta}$.}
\STATE {$\Sigma_{T_{-k}}\leftarrow A\Sigma_{S_k}A^T+I_d$.}
\STATE {$\Sigma_C\leftarrow [(\Sigma_x\!+\!(k-1)\Sigma_{\theta})A_1,\dots,(\Sigma_x\!+\!(k-1)\Sigma_{\theta})A_k/k]$}
\STATE {$\Sigma_{S_k|T_{-k}}\leftarrow\Sigma_{S_k}-\Sigma_C\Sigma_{T_{-k}}^{-1}\Sigma_C^T$}
\STATE {$\Sigma_{S_k|X,T_{-k}}\leftarrow\Sigma_{S_k}-[\Sigma_{\theta},\Sigma_C]\Sigma_{X,T_{-k}}^{-1}[\Sigma_{\theta},\Sigma_C]^T$.}
\STATE  {Compute $K$ and eigenvalues $\lambda_1,\lambda_2,\dots$ and left eigenvectors $v_1,v_2,\dots$}
\STATE  {Compute the projection matrix of each round, $A_i$ based on Theorem \ref{projection}.}
\STATE {Compute the critical values of $\beta$ for each eigenvalue as $\beta_c=\frac{1}{1-\lambda}$, and initiate value for $\beta_{size}$.} 
%\FOR{$\beta$ = $\beta_c:\beta_{size}$ \do }
%\STATE \begin{equation}\begin{aligned}
%  &R(\beta) = \frac{1}{2}\sum_{i=1}^{n(\beta)} \log\left((\beta-1)\frac{1-\lambda_i}{\lambda_i} \right) \\
%  &I(X;T_k|T_{-k})_{\beta} = \frac{1}{2}\sum_{i=1}^{n(\beta)} \log\left(\lambda_i \frac{\beta}{\beta - 1}\right)\nonumber
%\end{aligned}
%\end{equation}
%\ENDFOR
\STATE {$A=diag(A_1,\dots,A_k)$}
\ENDFOR
\end{algorithmic}
\end{algorithm}
\noindent
where $\beta_{size}$ determines the rank of the projection matrix in each round and depends on the $\beta_c$. In this algorithm, first, for each round (from 1 to $N$) we find the matrix $K$ and its eigenvalues and eigenvectors. Then, we compute the projection matrix $A_k$ of this round according to $\beta_{size}$ and the eigenvalues and eigenvectors of the matrix $K$ and save it to calculate the $K$ for the next round.\par 
Similar to the batch dataset, from the sufficiency of the sample mean $S_k$, we see that regardless of $k$, the optimum compression of each round $T_k$ is a $d$-dimensional representation of the  training set $X^k$; however, in our algorithm the global projection matrix $A$ is a $dk$-dimensional diagonal matrix operator, which we need it to compute the $\Sigma_{T_{-k.}}$. In general, in this problem one can derive the optimum operator from the $d$-dimensional matrix $K$ and compute the projection matrix $A_k$ in each round  and store it into the $A=diag(A_1,\dots,A_k)$. \par
 \begin{figure}[htb]
\centering
  \includegraphics[width=7cm]{CompareStream.pdf}
\caption {Compare online and comprehensive solution.}
\label{fig:Compare_Stream}
\end{figure}
Furthermore, we solve this optimization problem for $k=2$ using numerical optimization methods for scalar case. Figure.~\ref{fig:Compare_Stream} shows that the comprehensive solution is the optimum solution and converges to the GIB solution, in which we use the all rate in the last round, while the online solution is strictly sub-optimum. \par
%\setlength\belowcaptionskip{-2.5ex}
 \begin{figure}[htb]
\centering
  \includegraphics[width=7cm]{DisSamplesDifRates.pdf}
\caption {Number of Samples-Distortion curve for jointly Gaussian distribution with $d=10$ and $R\in\{4,8,10,14,16\}$.}
\label{fig:Rate-RelStream}
\end{figure}
In Figure \ref{fig:Rate-RelStream} we show the sample-distortion curve for a jointly Gaussian distribution, where $h(X|\theta)$ and $k$ represent the distortion function and the number of rounds or the number of samples that we use, receptively. In addition, for a fixed rate, as the number of samples increase we see that the distortion decreases; however, for a sufficiently large number of samples, this reduction becomes negligible. This can be interpreted as the eigenvalue of the $K$ matrix tends to 1.
%\begin{thebibliography}{9}
%\bibitem{GIB}
%Chechik, G. A. (2005). Information bottleneck for Gaussian variables. Journal of Machine Learning Research 6, 165-188.
%\end{thebibliography}
%\end{document}
%for every $\overline{X}_k$ and $T_k$  with jointly Gaussian distribution, we can represent the linear transformation 

 %In addition, the Markov chain is now $X-\theta-S_k-T_k$. 
%As reference \cite{chechik2005information}shows that the IB-optimum compression is $T_k = AS_k + Z$, where $Z$ is white Gaussian noise and $A$ is a matrix whose rows are scaled left eigenvectors of the matrix
